Mesoscopic Insights: Orchestrating Multi-scale & Hybrid Architecture for Image Manipulation Localization

The mesoscopic level serves as a bridge between the macroscopic and microscopic worlds, addressing gaps overlooked by both. Image manipulation localization (IML), a crucial technique to pursue truth from fake images, has long relied on low-level (microscopic-level) traces. However, in practice, most tampering aims to deceive the audience by altering image semantics. As a result, manipulation commonly occurs at the object level (macroscopic level), which is equally important as microscopic traces. Therefore, integrating these two levels into the mesoscopic level presents a new perspective for IML research. Inspired by this, our paper explores how to simultaneously construct mesoscopic representations of micro and macro information for IML and introduces the Mesorch architecture to orchestrate both. Specifically, this architecture i) combines Transformers and CNNs in parallel, with Transformers extracting macro information and CNNs capturing micro details, and ii) explores across different scales, assessing micro and macro information seamlessly. Additionally, based on the Mesorch architecture, the paper introduces two baseline models aimed at solving IML tasks through mesoscopic representation. Extensive experiments across four datasets have demonstrated that our models surpass the current state-of-the-art in terms of performance, computational complexity, and robustness.

==> sec/7_checklist.tex <==
\section{Reproducibility Checklist}
\begin{enumerate}
    \item This paper:
    \begin{enumerate}
        \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
        \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
        \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
    \end{enumerate}

    \item Does this paper make theoretical contributions? (yes)
    \begin{enumerate}
        \item All assumptions and restrictions are stated clearly and formally. (yes)
        \item All novel claims are stated formally (e.g., in theorem statements). (yes)
        \item Proofs of all novel claims are included. (yes)
        \item Proof sketches or intuitions are given for complex and/or novel results. (yes)
        \item Appropriate citations to theoretical tools used are given. (yes)
        \item All theoretical claims are demonstrated empirically to hold. (yes)
        \item All experimental code used to eliminate or disprove claims is included. (yes)
    \end{enumerate}

    \item Does this paper rely on one or more datasets? (yes)
    \begin{enumerate}
        \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
        \item All novel datasets introduced in this paper are included in a data appendix. (yes)
        \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
        \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes)
    \end{enumerate}

    \item Does this paper include computational experiments? (yes)
    \begin{enumerate}
        \item Any code required for pre-processing data is included in the appendix. (yes).
        \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)
        \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
        \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
        \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
        \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
        \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
        \item This paper states the number of algorithm runs used to compute each reported result. (yes)
        \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
        \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
        \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
        \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)
    \end{enumerate}

 
\end{enumerate}
